Too Large; Data Reduction for Vision-Language Pre-Training

This paper examines the problems of severe image-text misalignment and high redundancy in the widely-used large-scale Vision-Language Pre-Training (VLP) datasets. To address these issues, we propose an efficient and straightforward Vision-Language learning algorithm called TL;DR, which aims to compress the existing large VLP data into a small, high-quality set. Our approach consists of two major steps. First, a codebook-based encoder-decoder captioner is developed to select representative samples. Second, a new caption is generated to complement the original captions for selected samples, mitigating the text-image misalignment problem while maintaining uniqueness. As the result, TL;DR enables us to reduce the large dataset into a small set of high-quality data, which can serve as an alternative pre-training dataset. This algorithm significantly speeds up the time-consuming pretraining process. Specifically, TL;DR can compress the mainstream VLP datasets at a high ratio, e.g., reduce well-cleaned CC3M dataset from 2.82M to 0.67M ($\sim$24\%) and noisy YFCC15M from 15M to 2.5M ($\sim$16.7\%). Extensive experiments with three popular VLP models over seven downstream tasks show that VLP model trained on the compressed dataset provided by TL;DR can perform similar or even better results compared with training on the full-scale dataset. The code will be made available at \url{https://github.com/showlab/datacentric.vlp}.

==> figures/cluster_sample_ration_abl.tex <==
\begin{figure}[h]
  \centering
    \includegraphics[width=\linewidth]{figures/src/sampling_ratio_cluster_abl.png}
   \caption{
   }
   \label{fig:4_sampling_ratio_cluster_abl}
\end{figure}






==> tables/captioning.tex <==
\begin{table*}[h]
	\centering	
		\caption
	{
	%\small	
	\textbf{The image captioning results on NoCaps and COCO Caption.}
    This task require a text decoder which is missed in ViLT and CLIP so we only report BLIP architecture.
	C: CIDEr, S: SPICE, B@4: BLEU@4.	
	}
    %\setlength\tabcolsep{5pt}
	\resizebox{\textwidth}{!}{%
	\begin{tabular}	{l l  l |  l l l l l l l l | l l }	 	
	   \multirow[t]{3}{*}{Method}& \multirow[t]{3}{*}{{ Dataset}} & Samples &  \multicolumn{8}{c|}{ NoCaps validation} & 
	 \multicolumn{2}{c}{ COCO Caption}\\
	 && & \multicolumn{2}{c}{in-domain} & \multicolumn{2}{c}{near-domain} & \multicolumn{2}{c}{out-domain} & \multicolumn{2}{c|}{Overall} & \multicolumn{2}{c}{Karpathy test}\\
	 && & CIDEr & SPICE & CIDEr & SPICE & CIDEr & SPICE & CIDEr & SPICE & B@4 & CIDEr\\
	  \shline
       \hline
       \multirow{2}{*}{BLIP~\cite{blip}} & \CCThree~\cite{cc3m}&\\
       &\ModelNameCCThree&&&\\
       	   \multirow{2}{*}{BLIP~\cite{blip}} & \CCThree~\cite{cc3m} &155M&79.6 & 12.3 & 66.1 & 11.5 & 45.3 & 9.7 & 80.9 & 11.3 & 37.4 & 127.8 \\
	  &\ModelNameCCThree &347M& 103.1 & 14.2 & 96.1 & 13.8 & 88.3 & 12.1 & 95.5 & 13.5 &  38.2 & \bf 129.3 \\
	\end{tabular}
 	}
% \vspace{-2ex}
	\vspace{-1ex}
	\label{tab:caption}
\end{table*}		
